BadSampler: Harnessing the Power of Catastrophic Forgetting to Poison Byzantine-robust Federated Learning

Federated Learning (FL) is susceptible to poisoning attacks, wherein compromised clients manipulate the global model by modifying local datasets or sending manipulated model updates. Experienced defenders can readily detect and mitigate the poisoning effects of malicious behaviors using Byzantine-robust aggregation rules. However, the exploration of poisoning attacks in scenarios where such behaviors are absent remains largely unexplored for Byzantine-robust FL. This paper addresses the challenging problem of poisoning Byzantine-robust FL by introducing catastrophic forgetting. To fill this gap, we first formally define generalization error and establish its connection to catastrophic forgetting, paving the way for the development of a clean-label data poisoning attack named BadSampler. This attack leverages only clean-label data (i.e., without poisoned data) to poison Byzantine-robust FL and requires the adversary to selectively sample training data with high loss to feed model training and maximize the model's generalization error. We formulate the attack as an optimization problem and present two elegant adversarial sampling strategies, Top-$\kappa$ sampling, and meta-sampling, to approximately solve it. Additionally, our formal error upper bound and time complexity analysis demonstrate that our design can preserve attack utility with high efficiency. Extensive evaluations on two real-world datasets illustrate the effectiveness and performance of our proposed attacks.

==> eq3.tex <==
\begin{equation}\label{eq-3}
\vspace{-0.5cm}
                \mathop {\min }\limits_\omega f(\omega ),{\text{where}}\text{ }f(\omega ): = \sum\limits_{k = 1}^K {{p_k}{F}_k(\omega)},
\end{equation}
where ${p_k} \geqslant 0,\sum\nolimits_k {{p_k} = 1} $ is a user-defined term which indicates the relative influence of each client on the global model. In Eq. \eqref{eq-3}, we mainly focus on the \emph{local optimization} term which determines the performance of the global model. In fact, this local optimization term can be regarded as solving a \emph{non-convex optimization problem} with respect to the parameter $\omega^k$, corresponding to minimization of a given local loss function $F_k(\omega^k;x)$. For the $k$-th client, we assume that the batch size of local training is $B$ and let $N \cdot  B$ be the total number of items for training, then in a single epoch one aims to optimize: ${F_k}({\omega ^k};x) = \frac{1}{N}\sum\nolimits_{i = 1}^N {{\ell _i}(} {\omega ^k};{x_i})$. In general, we use the stochastic gradient descent (SGD) algorithm to solve the above optimization problem, \ie, the following weight update rule is implemented in a training epoch: 
$\omega _{t + 1}^k = \omega _t^k + \eta \Delta \omega _t^k,\Delta \omega _t^k =  - {\nabla _\omega }\ell ({\omega ^k};x),$ where $\eta$ is the learning rate.

%\mathop {\min }\limits_\omega  f(\omega ),{\text{ where} f(\omega ): = \sum\limits_{k = 1}^K {{p_k}{F_k}(\omega ;x)} ,

==> eq5.tex <==

 %As shown in Eq. \eqref{eq-5}, the stochastic error corresponding to the second-order correction term depends on the local training batch provided by the local sampler. Therefore, our poisoning attack aims to produce a sequence of poisoned training batches such that the first and second derivatives are misaligned with the true gradient step size by manipulating the local sampler. From federated optimization and batching, we find that model behavior can be influenced by observing and copying local training batches that produce gradients or model updates that are detrimental to global model training. As a result, we advocate the selection of local training batches which are not conducive to model training, \ie, ``bad batch'', and encourage the model to over-memorize the features mapped by the bad batch, forcing the model to forget generalizable features. 
%\vspace{-0.4cm}

